Learning to Map Context-Dependent Sentences to Executable Formal Queries

We propose a context-dependent model to map utterances within an interaction to executable formal queries. To incorporate interaction history, the model maintains an interaction-level encoder that updates after each turn, and can copy sub-sequences of previously predicted queries during generation. Our approach combines implicit and explicit modeling of references between utterances. We evaluate our model on the ATIS flight planning interactions, and demonstrate the benefits of modeling context and explicit references.

==> data.tex <==
\section{Data}
\as{Talk about data format}
\as{Date resolution and how we did it, plus accuracy of UWTime}
\as{Anonymization plus lookup tables generated from the schema}
\as{Snippets?}
\as{data statistics, e.g., number of utterances per interaction, length of utterances, length of SQL queries, vocabulary size...}
